Continuous PDE Dynamics Forecasting with Implicit Neural Representations

Effective data-driven PDE forecasting methods often rely on fixed spatial and / or temporal discretizations. This raises limitations in real-world applications like weather prediction where flexible extrapolation at arbitrary spatiotemporal locations is required. We address this problem by introducing a new data-driven approach, DINo, that models a PDE's flow with continuous-time dynamics of spatially continuous functions. This is achieved by embedding spatial observations independently of their discretization via Implicit Neural Representations in a small latent space temporally driven by a learned ODE. This separate and flexible treatment of time and space makes DINo the first data-driven model to combine the following advantages. It extrapolates at arbitrary spatial and temporal locations; it can learn from sparse irregular grids or manifolds; at test time, it generalizes to new grids or resolutions. DINo outperforms alternative neural PDE forecasters in a variety of challenging generalization scenarios on representative PDE systems.

==> tables/results_temporal_ablation.tex <==
\begin{wraptable}[9]{hR}{0.43\textwidth} \vspace{-0.3cm}
    \centering
    \caption{\textbf{Finer time resolution}: \textit{test} MSE ($\downarrow$) at finer test resolution for \textit{Navier-Stokes}.\label{tab:temp_superresol}}
    \sisetup{detect-weight, table-align-uncertainty=true, table-number-alignment=center, output-exponent-marker = \textsc{e}, table-format=1.3e-1, exponent-product={}, retain-zero-exponent, mode=text}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lSS}
             \toprule
             Model & {\textit{In-t}} & {\textit{Out-t}} \\
             \midrule
             I-\ours (linear) & 3.459e-04 & 5.598e-04 \\
             I-\ours (quadratic) & 2.165e-04 & 4.473e-04 \\
             \ours (ODE solve) & \B 2.151e-04 & \B 4.388e-04 \\
             \bottomrule
        \end{tabular}}
\end{wraptable}

